Equilibrium States of Galactic Atmospheres II: Interpretation and Implications

The scaling of galaxy properties with halo mass suggests that feedback loops regulate star formation, but there is no consensus yet about how those feedback loops work. To help clarify discussions of galaxy-scale feedback, Paper I presented a very simple model for supernova feedback that it called the minimalist regulator model. This followup paper interprets that model and discusses its implications. The model itself is an accounting system that tracks all of the mass and energy associated with a halo's circumgalactic baryons--the central galaxy's atmosphere. Algebraic solutions for the equilibrium states of that model reveal that star formation in low-mass halos self-regulates primarily by expanding the atmospheres of those halos, ultimately resulting in stellar masses that are insensitive to the mass-loading properties of galactic winds. What matters most is the proportion of supernova energy that couples with circumgalactic gas. However, supernova feedback alone fails to expand galactic atmospheres in higher-mass halos. According to the minimalist regulator model, an atmospheric contraction crisis ensues, which may be what triggers strong black-hole feedback. The model also predicts that circumgalactic medium properties emerging from cosmological simulations should depend largely on the specific energy of the outflows they produce, and we interpret the qualitative properties of several numerical simulations in light of that prediction.

==> Generality_1Nov2023.tex <==
\section{Generality}
\label{sec:Generality}

Here we step back from the minimalist regulator model to consider the generality of its physical implications. According to our analysis: 
\begin{enumerate}
    \item A halo's stellar baryon fraction becomes nearly independent of $\eta_M$ if cumulative feedback energy input into the atmosphere significantly exceeds cumulative radiative losses.
%    \item Raising $\eta_M$ boosts an atmosphere's equilibrium ratio of radiative losses to feedback energy input.
    \item Lowering a galaxy's ratio of star formation to gas supply ($\dot{M}_*/\dot{M}_{\rm in}$) by boosting $\eta_M$ can increase its equilibrium star formation rate.
\end{enumerate}
These inferences may appear surprising, but how generally do they apply?

\subsection{Independent Stellar Baryon Fraction}
\label{sec:Independent}

Both inferences are based on an accounting framework (presented in \S \ref{sec:Dynamics}) that simply sorts a halo's baryonic mass and energy into categories and tracks how they move from one category to another. It makes few astrophysical assumptions and broadly applies to galactic baryon cycles dominated by supernova feedback. Adding a feedback term accounting for black-hole energy injection would make it even more general.

Section \S \ref{sec:Expansion} then adds an implicit restriction, because it assumes that gas ejected from a halo's central galaxy shares its energy with the rest of the galaxy's atmosphere. If that assumption is valid, then supernova feedback can reduce the central galaxy's gas supply by raising $E_{\rm CGM}$. In that case, the central galaxy's stellar mass depends primarily on the feedback energy input
\begin{equation}
    \eta_E \varepsilon_{\rm SN} M_* \sim M_{\rm CGM} v_{\rm c}^2
\end{equation}
needed to significantly reduce $\dot{M}_{\rm in}$ by lifting atmospheric gas. The equilibrium star formation rate that results is therefore generally insensitive to $\eta_M$. 

However, the energy-sharing assumption does not apply to an atmosphere supported by what we will call \textit{ballistic circulation}. In the purely ballistic limit, supernova feedback ejects gas in clumps that follow ballistic trajectories and do not share their energy with accreting gas or the ambient atmosphere. Supernova feedback then does not reduce the galaxy's gas supply. Section \S \ref{sec:Ballistic} discusses how $\eta_M$ affects $\dot{M}_*$ in that limit.
\\

\marknotes{Compare predicted $f_*$--$v_{\rm c}^2$ relations with observations and discuss relationship between Carr et al. and this paper's model}
\\

\subsection{Increased Star Formation}
\label{sec:IncreasedSF}

Whether or not a galaxy's equilibrium star formation rate increases as $\eta_M$ rises depends on whether its atmosphere has the property
\begin{equation}
    \frac {\partial} {\partial \eta_M} 
        \frac {\dot{M}_{\rm in} (\varepsilon_{\rm eq})} {1 + \eta_M} > 0
        \label{eq:RiseCriterion}
        \; \; .
\end{equation}
The partial derivative is positive for the generic atmosphere model of \S \ref{sec:GenericModel} because raising $\eta_M$ lowers $\varepsilon_{\rm eq}$ and $\dot{M}_{\rm in}$ depends exponentially on $-\varepsilon_{\rm eq}$. 

Figure \ref{fig:fstar_asy_multi_plot} shows that the sensitivity of star formation to $\eta_M$ sets in as $\varepsilon_{\rm eq}$ drops below $\varepsilon_{\rm acc}$ into the contracted regime in which $\varepsilon_{\rm eq} \approx \eta_E \varepsilon_{\rm SN} / ( 1 + \eta_M)$. In that regime, the criterion in equation (\ref{eq:RiseCriterion}) approximately reduces to
\begin{equation}
        \frac {\eta_E \varepsilon_{\rm SN}} {\eta_M}
        \: \gtrsim \: v_{\rm c}^2
\end{equation}
implying that raising $\eta_M$ increases the galaxy's equilibrium star formation rate as long as
the specific energy of ejected gas
\begin{equation}
    \varepsilon_{\rm ej} \equiv \frac {\eta_E \varepsilon_{\rm SN}} {\eta_M}
\end{equation} 
significantly exceeds $v_{\rm c}^2$. However, the generic model itself does not provide a clear physical interpretation of this outcome.

A clearer picture emerges from considering the impact of recycling on $\dot{M}_*$ \citep[see also][]{Oppenheimer_2010MNRAS.406.2325O}. The relationship between $\dot{M}_*$ and $\eta_M$ generally depends on the number of times baryons can cycle through a galaxy, which we will represent with the parameter $N_{\rm cyc}$. Suppose $\dot{M}_{\rm in,0}$ is the rate at which baryons enter a galaxy for the first time. The galaxy's time-averaged star formation rate is then roughly
\begin{align}
    \langle \dot{M}_* \rangle
        \: &\sim \: \frac {\dot{M}_{\rm in,0}} {1 + \eta_M}
                        \sum_{n = 0}^{N_{\rm cyc}}
                            \left( \frac {\eta_M} {1 + \eta_M} \right)^n
\end{align}
if $t_{\rm SF}$ is short enough to limit accumulation of incoming gas in the interstellar medium. 

Increasing $\eta_M$ reduces the probability that baryons form stars during a single cycle through the galaxy but can increase the number of cycles. The galaxy's star-formation rate is therefore $\sim \dot{M}_{\rm in,0} / (1 + \eta_M)$ for $N_{\rm cyc} \ll 1$. It is $\sim [ N_{\rm cyc} / (1 + \eta_M)] \dot{M}_{\rm in,0}$ for $1 \lesssim N_{\rm cyc} \ll \eta_M$. And it levels off at $\dot{M}_{\rm in,0}$ as $N_{\rm cyc}$ surpasses $\eta_M$. Atmospheres with the property
\begin{equation}
    \frac {\partial} {\partial \eta_M} \frac {N_{\rm cyc}} {1 + \eta_M} > 0
    \label{eq:NcycCriterion}
\end{equation}
consequently sustain equilibrium star formation rates that increase as $\eta_M$ rises when recycling dominates the gas supply.

\subsection{Ballistic Circulation}
\label{sec:Ballistic}

This section considers a schematic ballistic circulation scenario that satisfies the criterion in equation (\ref{eq:NcycCriterion}) under certain conditions but rests on a foundation different from the other models discussed in this paper. Instead of assuming that supernova feedback reduces a galaxy's gas supply by transferring some of its energy to the rest of the circumgalactic atmosphere, it assumes that ejected gas transfers little to none of its ejection energy. In that case, clumps of ejected gas follow nearly ballistic trajectories, reaching a maximum altitude determined by the specific energy $\varepsilon_{\rm ej}$ they had upon leaving the galaxy before falling back down toward it.\footnote{Some astronomers call this feedback mode ``juggling."}

Ejected gas cannot formally escape the isothermal potential well we have adopted, because $\varphi (r)$ logarithmically approaches infinity as $r$ increases. However, gas ejected with a specific energy much greater than the halo's accretion energy does not fall back down on a timescale short enough to be recycled. Consequently, there is a critical value of $\eta_M$ above which ballistic gas is recycled and below which it decouples from the galaxy's gas supply.

Small values of $\eta_M$ allow ballistic ejection to limit galactic star formation as long as $\varepsilon_{\rm ej}$ exceeds $\varepsilon_{\rm acc}$. That is because the specific energy of accreting gas is similar to the specific energy of ballistic gas that would return to the galaxy on a timescale similar to the universe's current age. The galaxy's star formation rate $\dot{M}_* \approx \dot{M}_{\rm in} / (1 + \eta_M)$ therefore declines with increasing $\eta_M$ while
\begin{equation}
    \eta_M \: \lesssim \: \frac {\eta_E \varepsilon_{\rm SN}} {\varepsilon_{\rm acc}}
\end{equation}
because feedback does not lower the galaxy's gas supply rate $\dot{M}_{\rm in}$. However, greater values of $\eta_M$ promote recycling that raises $\dot{M}_{\rm in}$ and can boost the galaxy's star formation rate. 

The number of times a ballistic particle can pass through a halo's central galaxy depends inversely on the ballistic recycling timescale 
\begin{equation}
    t_{\rm ball} \: \equiv \: 
        2 \int_0^{v_{\rm ej}} \frac {r} {v_{\rm c}^2} \, dv
\end{equation}
associated with radial ejection at a speed $v_{\rm ej}$. If $t_{\rm ball}$ is significantly shorter than the age of the universe, then the number of cycles scales as $N_{\rm cyc} \propto t_{\rm ball}^{-1}$. Ballistic recycling with the property
\begin{equation}
    \frac {\partial \ln N_{\rm cyc}} {\partial \eta_M} 
      \: = \: - \frac {\partial \ln t_{\rm ball}} {\partial \eta_M} 
      \: > \: \frac {1} {1 + \eta_M}
\end{equation}
therefore results in an equilibrium star formation rate that rises as $\eta_M$ increases.

In a nearly isothermal potential well, the ballistic recycling timescale is approximately proportional to the maximum radius of a ballistic trajectory with specific energy $\eta_E \varepsilon_{\rm SN} / \eta_M$:
\begin{equation}
    r_{\rm ej} \approx r_0 \exp \left( \frac {\varepsilon_{\rm ej}}
                                            {v_{\rm c}^2} \right)
        \; \; .
\end{equation}
Taking the derivative of the expression for $r_{\rm ej}$ gives
\begin{equation}
    - \frac {\partial \ln t_{\rm ball}} {\partial \eta_M} 
        \: \approx \: - \frac {\partial \ln r_{\rm ej}} {\partial \eta_M}
        \: \approx \: \frac {\varepsilon_{\rm ej}} {\eta_M v_{\rm c}^2}
        \; \; .
\end{equation}
Mass loading factors rising through the range
\begin{equation}
    \frac {\eta_E \varepsilon_{\rm SN}} {\varepsilon_{\rm acc}} 
        \: \lesssim \: \eta_M 
        \: \lesssim \: \frac {\eta_E \varepsilon_{\rm SN}} {v_{\rm c}^2} 
\end{equation}
therefore increase the equilibrium star formation rate of a galaxy regulated by ballistic circulation. 
